Index theory on the Mi\v{s}\v{c}enko bundle

We consider the assembly map for principal bundles with fiber a countable discrete group. We obtain an index-theoretic interpretation of this homomorphism by providing a tensor-product presentation for the module of sections associated to the Mi\v{s}\v{c}enko line bundle. In addition, we give a proof of Atiyah's $L^2$-index theorem in the general context of principal bundles over compact Hausdorff spaces. We thereby also reestablish that the surjectivity of the Baum-Connes assembly map implies the Kadison-Kaplansky idempotent conjecture in the torsion-free case. Our approach does not rely on geometric $K$-homology but rather on an explicit construction of Alexander-Spanier cohomology classes coming from a Chern character for tracial function algebras.

==> mathHeadings.tex <==
%*********************************************************************************
% Theorems, propositions, etc.
%*********************************************************************************
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]

\newtheorem{theoremA}{Theorem}[section]
\renewcommand*{\thetheoremA}{\Alph{theoremA}}

\newtheorem*{theorem*}{Theorem}
\newtheorem*{corollary*}{Corollary}
\newtheorem*{conjecture*}{Conjecture}
\newtheorem*{question*}{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition} 
\newtheorem{definition}[theorem]{Definition}

%*******************************
% Jens's settings
%*******************************
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[theorem]{Proposition}
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{cor}[theorem]{Corollary}
%\newtheorem{defprop}[theorem]{Definition and Proposition}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\newtheorem{assu}[theorem]{Assumption}

\theoremstyle{definition}
\newtheorem{dfn}[theorem]{Definition}

%\theoremstyle{remark} % i.e. same as plain, but theorembodyfont is rm

%\newtheorem{example}[theorem]{Example}
%\newtheorem{examples}[theorem]{Examples}
%\newtheorem{remark}[theorem]{Remark}

==> mathMacros.tex <==
%*********************************************************************************
% Math macros
%*********************************************************************************
\newcommand{\numberset}{\mathbb} 
\newcommand{\N}{\numberset{N}} 
\newcommand{\Z}{\numberset{Z}} 
\newcommand{\Q}{\numberset{Q}} 
\newcommand{\R}{\numberset{R}}
\let\C\relax
\newcommand{\C}{\numberset{C}}
\newcommand{\Cc}{\numberset{C}}
%\let\T\relax
%\let\M\relax
%\newcommand{\T}{\mathrm{T}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Cast}{$C^\ast$}
\DeclareMathOperator{\Chern}{Ch}
\DeclareMathOperator{\HC}{HC}
\DeclareMathOperator{\HP}{HP}
%\DeclareMathOperator{\ab}{ab}
\DeclareMathOperator{\RK}{RKK}
\DeclareMathOperator{\KKK}{KK}
\DeclareDocumentCommand{\KK}{O{*} O{} m m}{\KKK_{#1}^{#2}(#3,#4)}
%\DeclareMathOperator{\Trace}{Tr}
\newcommand{\hatotimes}{\widehat{\otimes}}
%\newcommand{\hot}{\widehat{\otimes}}
\newcommand{\Vn}{\mathcal{N}}

\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern.1pt\mathchar"0362\kern.1pt}%
    {\rule{0ex}{\textheight}}%WIDTH-LIMITED CIRCUMFLEX
  }{\textheight}% 
}{2.4ex}}%
\stackon[-6.9pt]{#1}{\tmpbox}%
}
\parskip 1ex

%*******************************
% Jens's settings
%*******************************
%\newcommand{\cd}{\cdot}
%\newcommand{\ced}{\centerdot}
%\newcommand{\clc}{\cdot\ldots\cdot}
%\newcommand{\ot}{\otimes}
%\newcommand{\od}{\odot}
%\newcommand{\hot}{\widehat \otimes}
%\newcommand{\wot}{\widetilde \otimes}
%\newcommand{\bt}{\bigotimes}
%%\newcommand{\op}{\oplus}
%\newcommand{\bop}{\bigoplus}
%\newcommand{\oplop}{\oplus \ldots \oplus}
%\newcommand{\olo}{\otimes\ldots\otimes}
%\newcommand{\plp}{+ \ldots +}
%\newcommand{\tlt}{\times \ldots \times}
%\newcommand{\we}{\wedge}
%\newcommand{\wlw}{\wedge\ldots\wedge}
%\newcommand{\glg}{\hat\otimes \ldots \hat\otimes}
%\newcommand{\calca}{\cap \ldots \cap}
%\newcommand{\ci}{\circ}
%\newcommand{\cilci}{\circ \ldots \circ}
%\newcommand{\ti}{\times}
%
%\newcommand{\nn}{\mathbb{N}}
%\newcommand{\zz}{\mathbb{Z}}
%\newcommand{\QQ}{\mathbb{Q}}
%\newcommand{\rr}{\mathbb{R}}
%\newcommand{\cc}{\mathbb{C}}
%\newcommand{\kk}{\mathbb{K}}
%\newcommand{\ff}{\mathbb{F}}
%
%\newcommand{\al}{\alpha}
%\newcommand{\be}{\beta}
%\newcommand{\ga}{\gamma}
%\newcommand{\Ga}{\Gamma}
%\newcommand{\de}{\delta}
%\newcommand{\De}{\Delta}
%\newcommand{\ep}{\varepsilon}
%\newcommand{\ph}{\varphi}
%\newcommand{\Ph}{\Phi}
%\newcommand{\io}{\iota}
%\newcommand{\ka}{\kappa}
%\newcommand{\la}{\lambda}
%\newcommand{\La}{\Lambda}
%\newcommand{\Na}{\nabla}
%\newcommand{\om}{\omega}
%\newcommand{\Om}{\Omega}
%\newcommand{\si}{\sigma}
%\newcommand{\Si}{\Sigma}
%\newcommand{\te}{\theta}
%\newcommand{\Te}{\Theta}
%\newcommand{\ze}{\zeta}
%
%\newcommand{\pa}{\partial}
%\newcommand{\da}{\dagger}
%\newcommand{\lf}{\lfloor}
%\newcommand{\rf}{\rfloor}
%\newcommand{\co}{\equiv}
%\newcommand{\ov}{\overline}
%%\newcommand{\C}[1]{\mathcal{#1}}
%%\newcommand{\G}[1]{\mathfrak{#1}}
%%\newcommand{\T}[1]{\textup{#1}}
%%\newcommand{\M}[1]{\mbox{#1}}
%%\newcommand{\E}[1]{\emph{#1}}
%%\newcommand{\B}[1]{\mathbb{#1}}
%%\newcommand{\F}[1]{\mathbf{#1}}
%%\newcommand{\OO}[1]{\operatorname{#1}}
%%\newcommand{\fork}[2]{\left\{ \begin{array}{#1} #2 \end{array} \right.} 
%%\newcommand{\arr}[2]{\begin{array}{#1}#2 \end{array}}
%%\newcommand{\ma}[2]{\left(\begin{array}{#1} #2 \end{array} \right)}
%%\newcommand{\arle}{\dgARROWLENGTH=0.5\dgARROWLENGTH}
%%\newcommand{\no}[1]{\node{#1}}
%%\newcommand{\ar}[2]{\arrow{#1}{#2}}
%\newcommand{\lrar}{\Leftrightarrow}
%\newcommand{\lar}{\Leftarrow}
%\newcommand{\rar}{\Rightarrow}
%\newcommand{\ex}{\exists}
%\newcommand{\su}{\subseteq}
%\newcommand{\ssu}{\supseteq}
%\newcommand{\sm}{\setminus}
%\newcommand{\es}{\emptyset}
%\newcommand{\q}{\qquad}
%\newcommand{\qq}{\qquad \qquad}
%\newcommand{\qqq}{\qquad \qquad \qquad}
%\newcommand{\qqqq}{\qquad \qquad \qquad \qquad}
%\newcommand{\wit}{\widetilde}
%\newcommand{\wih}{\widehat}
%\newcommand{\ft}[1]{{#1}^{\T{odd}}}
%\newcommand{\et}[1]{{#1}^{\T{ev}}}
%\newcommand{\fe}[1]{{#1}^{\E{odd}}}
%\newcommand{\ee}[1]{{#1}^{\E{ev}}}
%\newcommand{\deht}[2]{\T{det}\big(H_{#1}(#2)\big)}
%\newcommand{\dehe}[2]{\E{det}\big(H_{#1}(#2)\big)}
%\newcommand{\dht}[2]{\T{dim}\big(H_{#1}(#2) \big)}
%\newcommand{\dhe}[2]{\E{dim}\big(H_{#1}(#2) \big)}
%\newcommand{\hodht}[4]{\T{Hom}\Big( \T{det}\big(H_{#1}(#2) \big),
  %\T{det}\big(H_{#3}(#4) \big)\Big)}
%\newcommand{\diff}[2]{\frac{\partial{#1}}{\partial{#2}}}
%\newcommand{\dir}{\slashed{\C D}}
%\newcommand{\lap}{\slashed{\De}}
%\newcommand{\sla}[1]{\slashed{#1}}
%\newcommand{\inn}[1]{\langle #1 \rangle}
%\newcommand{\binn}[1]{\big\langle #1 \big\rangle}
%\newcommand{\cross}[1]{#1\rtimes_\alpha \mathbb{Z}}
%%\newcommand{\grad}{\hat\otimes}
%\newcommand{\gradodd}{\hat\otimes\varepsilon}
%\newcommand{\ovar}{\otimes_\varphi}
%\newcommand{\govar}{\hat\otimes_\varphi}
%\newcommand{\ho}{\C O(\Omega)}
%\newcommand{\hoc}{\C O\big(\T{Sp}(A)\big)}
%\newcommand{\spa}{\T{Sp}(A)}
%\newcommand{\spe}{\T{Sp}_{\T{ess}}(A)}
%\newcommand{\sem}{\setminus}

%******************
% fancy fonts
%******************
%\providecommand{\mathscr}{\mathcal} % a priori mathscr is mathcal
%\IfFileExists{mathrsfs.sty}{
%\usepackage{mathrsfs}}         %  \mathscr produces rsfs fonts
   %{%  else try euler fonts
     %\IfFileExists{eucal.sty}{
        %\usepackage[mathscr]{eucal}} % \mathscr produces Euscript fonts,
                     %% the option [mathscr] ensures that
                     %% \mathcal is not altered
   %{% else both unavailable, do nothing, mathscr remains mathcal
   %}
%}
%\newcommand\sA{\mathscr{A}}
%\newcommand\sB{\mathscr{B}}
%\newcommand\sC{\mathscr{C}}
%\newcommand\sD{\mathscr{D}}
%\newcommand\sE{\mathscr{E}}
%\newcommand\sF{\mathscr{F}}
%\newcommand\sG{\mathscr{G}}
%\newcommand\sH{\mathscr{H}}
%\newcommand\sI{\mathscr{I}}
%\newcommand\sJ{\mathscr{J}}
%\newcommand\sK{\mathscr{K}}
%\newcommand\sL{\mathscr{L}}
%\newcommand\sM{\mathscr{M}}
%\newcommand\sN{\mathscr{N}}
%\newcommand\sO{\mathscr{O}}
%\newcommand\sP{\mathscr{P}}
%\newcommand\sQ{\mathscr{Q}}
%\newcommand\sR{\mathscr{R}}
%\newcommand\sS{\mathscr{S}}
%\newcommand\sT{\mathscr{T}}
%\newcommand\sU{\mathscr{U}}
%\newcommand\sV{\mathscr{V}}
%\newcommand\sW{\mathscr{W}}
%\newcommand\sX{\mathscr{X}}
%\newcommand\sY{\mathscr{Y}}
%\newcommand\sZ{\mathscr{Z}}
